Automated Test Generation for Scratch Programs

The importance of programming education has lead to dedicated educational programming environments, where users visually arrange block-based programming constructs that typically control graphical, interactive game-like programs. The Scratch programming environment is particularly popular, with more than 70 million registered users at the time of this writing. While the block-based nature of Scratch helps learners by preventing syntactical mistakes, there nevertheless remains a need to provide feedback and support in order to implement desired functionality. To support individual learning and classroom settings, this feedback and support should ideally be provided in an automated fashion, which requires tests to enable dynamic program analysis. The Whisker framework enables automated testing of Scratch programs, but creating these automated tests for Scratch programs is challenging. In this paper, we therefore investigate how to automatically generate Whisker tests. This raises important challenges: First, game-like programs are typically randomised, leading to flaky tests. Second, Scratch programs usually consist of animations and interactions with long delays, inhibiting the application of classical test generation approaches. Evaluation on common programming exercises, a random sample of 1000 Scratch user programs, and the 1000 most popular Scratch programs demonstrates that our approach enables Whisker to reliably accelerate test executions, and even though many Scratch programs are small and easy to cover, there are many unique challenges for which advanced search-based test generation using many-objective algorithms is needed in order to achieve high coverage.

==> sections/experiments-old.tex <==
\begin{figure}[t]
	\subfloat[\label{fig:pingpong_stage}Ping Pong]{\includegraphics[width=0.3\textwidth]{figures/pingpong_stage}}
	\hfill
	\subfloat[\label{fig:fruit_stage}Fruit Catching]{\includegraphics[width=0.3\textwidth]{figures/fruit_stage}}
	\hfill
	\subfloat[\label{green_stage}Green Your City]{\includegraphics[width=0.3\textwidth]{figures/green_stage}}
	\\
	\subfloat[\label{fig:fruit_code}Code excerpt of the \\Fruit Catching game]{\includegraphics[trim=0 65 0 275,clip,width=0.35\textwidth]{figures/fruit_banana_code}}	
	\subfloat[\label{fig:green_code}Code excerpt of the Green Your City game]{\includegraphics[trim=0 80 0 50,clip,width=0.6\textwidth]{figures/green_code}}	
%	\subfloat[\label{fig:fruit_code}Code excerpt of the Fruit Catching game]{\includegraphics[trim=0 200 0 140,clip,width=0.32\textwidth]{figures/fruit_code}}	
	\\
	\subfloat[\label{fig:pingpong_code}Code excerpt of the Ping Pong game]{\includegraphics[trim=0 300 0 140,clip,width=\textwidth]{figures/pingpong_code}}
	
	\caption{\label{sec:examples}Case study programs and code examples.}
\end{figure}





 
To illustrate the proposed approach, we use three example \scratch programs
shown in \cref{sec:examples}. The Ping Pong game is a classical \scratch
tutorial example, and represents the types of programs commonly created by
early learners. It consists of 36 blocks in 4 scripts, and is controlled by
five different key events. We modified the Ping Pong game to initialise all
variables (missing variable initialisation is a common bug in
\scratch~\cite{fraedrich2020}). The Fruit Catching game was used by Stahlbauer
et al.~\cite{TestingScratch} as part of their evaluation of \whisker, and is
taken from an educational context. It consists of 49 blocks in 4 scripts, and
is controlled by the cursor keys. Green Your City is part of the popular CodeClub collection of example projects. It consists of 8 scripts and 52 blocks.

\FloatBarrier


\begin{figure}[t]
	\subfloat[\label{fig:banana1}Branch distance 284]{\includegraphics[width=0.31\textwidth]{figures/banana1}}
	\hfill
	\subfloat[\label{fig:banana2}Branch distance 188]{\includegraphics[width=0.31\textwidth]{figures/banana2}}
	\hfill
	\subfloat[\label{fig:banana3}Branch distance 87]{\includegraphics[width=0.31\textwidth]{figures/banana3}}	
	\caption{\label{fig:banana_distance}Fitness values for statements within the if-condition shown in \cref{fig:fruit_code}.  \\
	{\small The approach level is 0 in all cases, but the branch distance of the if-condition depends on the distance between the bowl and the banana.}}
\end{figure}

\begin{figure}[t]
	\subfloat[\label{fig:pingpong1}Branch distance 190]{\includegraphics[width=0.31\textwidth]{figures/pingpong1}}
	\hfill
	\subfloat[\label{fig:pingpong2}Branch distance 224]{\includegraphics[width=0.31\textwidth]{figures/pingpong2}}
	\hfill
	\subfloat[\label{fig:pingpong3}Branch distance 37]{\includegraphics[width=0.31\textwidth]{figures/pingpong3}}	
	\caption{\label{fig:pingpong_distance}Fitness values for statements within the first if-condition shown in \cref{fig:pingpong_code}.  \\
	{\small The approach level is 1 if $x > 225$ or $x < -225$, otherwise it is 0. Given that the ball faces in direction $-75$ (such that the branch distance for $-75 > 90$ is $90 - -75 + 1 = 166$, and the branch distance for $-75 > -90$ is $0$) and is between the paddles, the branch distance is calculated as $min(distance(ball, right\_paddle) + 166, distance(ball, left\_paddle) + 0))$.}}
	\vspace{-1em}
\end{figure}
 
\begin{figure}[t]
	\subfloat[\label{fig:green1}Branch distance 136]{\includegraphics[width=0.31\textwidth]{figures/green1}}
	\hfill
	\subfloat[\label{fig:green2}Branch distance 128]{\includegraphics[width=0.31\textwidth]{figures/green2}}
	\hfill
	\subfloat[\label{fig:green3}Branch distance 297]{\includegraphics[width=0.31\textwidth]{figures/green3}}	
	\caption{\label{fig:green_distance}Fitness values for statements within the first if-condition shown in \cref{fig:green_code}, which is duplicated for each flower. \\
	{\small The approach level is 0 if the green flag is clicked; the branch distance is calculated based on the $y$-position and the distance to the closest water drop. Given that a flower needs to be below $y = -150$, the branch distance for the flower in \cref{fig:green1} is $distance(flower, water) + (-129 - (-150) + 1) =  136$. The flower in \cref{fig:green2} is below $y = -150$, therefore the branch distance is $distance(flower, water) + 0 = 128$, and for \cref{fig:green3} it is 297.}}
	\vspace{-1em}
\end{figure}

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.8\textwidth]{figures/fruit_evolution}
% 	\caption{\label{fig:fruit_evolution}Example evolution (1+1 EA) for the fitness function of catching the banana (Code in \cref{fig:fruit_code}, fitness examples in \cref{fig:banana_distance}) and corresponding chromosomes. After the banana has been caught at iteration 15, the evolution continues shortening the test case down to pressing the right key three times, and then left two times.}
% 	\vspace{-1em}
% \end{figure}



\FloatBarrier

\begin{figure}[!t]
	\subfloat[\label{fig:result_pingpong}Ping Pong]{\includegraphics[width=0.33\textwidth]{generated_files/pingpong}}
	\hfill
	\subfloat[\label{fig:result_fruit}Fruit Catching]{\includegraphics[width=0.33\textwidth]{generated_files/fruit}}
	\hfill
	\subfloat[\label{fig:result_green}Green Your City]{\includegraphics[width=0.33\textwidth]{generated_files/green}}
	\caption{\label{fig:coverage}Coverage over time, averaged over 30 runs.}
\end{figure}

In a typical \scratch program, many statements are trivially covered, but there can always be tricky code that poses challenges for automated testing.  
\Cref{fig:fruit_code} shows an excerpt of the code of the Fruit Catching game, taken from the banana sprite: In order to execute the statements in the then-block of the shown branch, the player-controlled bowl needs to touch the banana. The \emph{touching} predicate is reflected by a branch distance that guides the test generator towards achieving this, as illustrated in \cref{fig:banana_distance} for different states of the game. %\Cref{fig:fruit_evolution} demonstrates the evolution for one coverage goal in the then-branch in terms of the fitness values and corresponding chromosomes.




The if-condition of the Ping Pong game shown in \cref{fig:pingpong_code} requires a branch distance calculation by applying the rules on nested logical expressions to combine the distances between the ball and the two paddles, as well as the required and current orientation of the ball. As suggested by the example states shown in \cref{fig:pingpong_distance}, the fitness landscape induced by the complex expression is less convenient than in the simple \emph{touching}-predicate shown in \cref{fig:banana_distance}. Green Your City also contains logical expressions combining various distance measurements; in particular each of the flowers contains the code shown in \cref{fig:green_code}. Flowers grow vertically each time they touch a water drop, the example branch is covered once this has happened sufficiently often to let the flower grow above $y = -150$ and it touches a water drop again; \cref{fig:green_distance} shows examples of this distance for different flowers.



To see the search in action, \Cref{fig:coverage} shows the coverage over time,
averaged over 30 runs of \whisker using the original
configuration~\cite{TestingScratch} (``Random'', i.e., \SI{60}{\second}, events every \SI{250}{\milli\second},
program reset every \SI{10}{\second}), and the search extension (``Search'', \SI{60}{\second} runtime,
population size 10, \SI{250}{\milli\second} default event duration, acceleration factor 5, crossover probability 0.8, initial length 2).
%
The improvement of the search over random testing after \SI{60}{\second} is statistically significant with $p < 0.001$ in all three cases: For Ping Pong the Vargha-Delaney effect size $\hat{A}_{12} = 0.7$, for the Fruit Catching game $\hat{A}_{12} = 1.0$, and for Green Your City $\hat{A}_{12} = 1.0$.
%
For Ping Pong (\cref{fig:result_pingpong}) the search covers most statements quickly, but generally needs longer ($\approx$\SI{30}{\second}) to cover the two branches discussed in example \cref{fig:pingpong_distance}. Random testing sometimes hits the ball by accident, but generally needs to play much longer before that happens. Similarly, for the Fruit Catching game \cref{fig:result_fruit} shows, while again many statements are easy to cover, the search needs about \SI{30}{\second} to succeed in catching both types of fruit, while random takes substantially longer.
%
The results for Green Your City (\cref{fig:result_green}) are similar, in that the search requires around \SI{30}{\second} until all statements are covered, while random usually takes longer; the tricky branches are those requiring to hit flowers with water drops, as well as one statement that requires the helicopter to reach the bottom, and thus a longer play time than random testing used would be necessary. While these are promising initial results, a more thorough evaluation on a larger number of \scratch projects is planned as future work. The randomised and game-like nature of most \scratch projects can be a cause for test flakiness; however, this flakiness can be easily contained~\cite{TestingScratch}.

Note that an automatically generated coverage test suite is only one of the stepping stones towards providing automated feedback to learners: The generated tests tend to be short and their randomised nature potentially makes them difficult to understand, and so we do not expect that the tests would be shown \emph{directly} to learners. The tests are rather meant as input to further dynamic analysis tools, for example in order to serve as test harness for \whisker~\cite{TestingScratch}, where manually written \scratch observers would provide insight into which aspects of the functionality are correctly implemented in a concrete learner's implementation of a predefined programming challenge. We envision that the concrete feedback to learners will be provided in terms of textual hints or code suggestions~\cite{price2017isnap,techapalokul2019code}, and the generated tests are a prerequisite for achieving this.



==> sections/experiments/event-selection.tex <==

\subsubsection{RQ3: What are the effects of event selection strategies?}
\label{subsec:experiment-event-selection}

\Cref{sec:event-selection} introduced three different strategies to extract
available events from \Scratch programs: A baseline approach of using all
events supported by \Scratch, a static approach considering the source code of
the program, and a dynamic approach also considering the execution state. Since
the event selection is orthogonal to the test generation algorithm applied, we
first establish the effects of the improved event selection techniques over the
baseline. In order to compare the event selectors independently of the used search algorithm, each event selector is combined with a random test generation approach, as explained in \Cref{sec:event-selection}, and applied to all projects of the \rand
and \topp datasets using a search budget of \SI{10}{\minute}. Furthermore, to reduce the inherent effect of randomness, the experiment on both datasets is repeated 30 times,
leading to 180,000 \whisker executions. We compare the selection techniques based on the average achieved block coverages across all projects. Moreover for each event selection combination,
we report on a per-project basis the \atwelve value and the number of projects for which a given approach obtained significantly more, more, equal, fewer and significantly fewer block coverage than another one.
Statistically significant results are determined using the Mann-Whitney-U test and a \pval smaller than 0.05.


==> sections/methods/search/operators.tex <==
\subsubsection{Search Operators}

Since the optimal number of events in a test case is problem specific and cannot be known ahead of time, we use a variable length encoding. This also provides an opportunity for the search to minimise the length of the tests.
%, such that users receive shorter tests with less redundancy.
%
To generate a random individual for the initial population we select a random length $n$ in the range $[1..max]$, where $max$ is a predetermined parameter representing the maximum number of events in a test case. Then, we generate $n$ random codons, each of which is selected from the range from $0$ to $480$;
the value $480$ is the width of the stage in pixels and thus the largest possible parameter any of our supported events can take.
%
The mutation operator can probabilistically (1) replace codons with random codons, (2) insert new codons, and (3) delete codons, each with a certain probability dependent on the length. 
%
The crossover operator splits the two parent chromosomes into two parts at a randomly selected relative point (i.e., $[0..1]$). Then the codons on the right side of that splitting point are swapped between the chromosomes. 
%
The mutation and crossover operators are based on prior work on variable size search~\cite{fraser2012whole} with the aim of avoiding test length bloat~\cite{fraser2013handling}. 

==> sections/methods/search/random-testing.tex <==
\subsection{Random Testing}


The most basic algorithm to derive a test suite is to repeatedly generate
random test cases. This may quickly lead to very large test suites, where many
tests do not contribute to our overall objective of achieving coverage.
Therefore, in order to prevent that test suites become excessively large, we
execute each newly generated test to measure its coverage, and only retain it
if it succeeds in covering at least one statement that no previous test had
covered. \Cref{alg:random_suite} describes this random test suite generation
procedure.

